Context2Name: A Deep Learning-Based Approach to Infer Natural Variable Names from Usage Contexts

Most of the JavaScript code deployed in the wild has been minified, a process in which identifier names are replaced with short, arbitrary and meaningless names. Minified code occupies less space, but also makes the code extremely difficult to manually inspect and understand. This paper presents Context2Name, a deep learningbased technique that partially reverses the effect of minification by predicting natural identifier names for minified names. The core idea is to predict from the usage context of a variable a name that captures the meaning of the variable. The approach combines a lightweight, token-based static analysis with an auto-encoder neural network that summarizes usage contexts and a recurrent neural network that predict natural names for a given usage context. We evaluate Context2Name with a large corpus of real-world JavaScript code and show that it successfully predicts 47.5% of all minified identifiers while taking only 2.9 milliseconds on average to predict a name. A comparison with the state-of-the-art tools JSNice and JSNaughty shows that our approach performs comparably in terms of accuracy while improving in terms of efficiency. Moreover, Context2Name complements the state-of-the-art by predicting 5.3% additional identifiers that are missed by both existing tools.

==> conclusion.tex <==
\section{Conclusion}

==> evaluation.tex <==
\section{Evaluation}

\ksen{This section should be the focus of Rohan.  It should be expanded and completed as soon as possible.}

To evaluate and compare our tool with existing techniques, we use a publicly available corpus containing 150,000 clear-text JS programs \cite{Raychev2016}. Of these, we use 100,000 files for training, and keep the other 50,000 files aside for evaluation. We train all the techniques on the same set of files so as to gauge the effectiveness of each tool. Accuracy is measured as the number of original names recovered \emph{exactly} from the minified files. Note that this metric of accuracy gives us a lower-bound on the effectiveness of any technique, as the predicted name may be very similar to, or even better than the original. We choose this metric as its computation can be automated. A manual evaluation of the quality of the names suggested is beyond the scope of this work.

\subsection{Setup}\label{sec-evaluation-setup}
\textbf{Corpus :} 
We use the publicly available dataset \cite{Raychev2016} comprising of 150,000 clear-text non-minified JavaScript files. The dataset also consists of a list of 100,000 files   to be used for training, and another list of 50,000 files to be used for testing. We removed all the files which had syntax errors and/or could not be processed by the minifier, which left us with 95826 files for training, and 47776 files for testing.\\

\noindent\textbf{Training :}
The training phase is straightforward and summarized in the previous section (Sec. \ref{sec-impl-training}). The values of the various parameters in our network used for training is provided in table \ref{tab:network-params}.\\

\noindent\textbf{Testing :} We first minify the files set aside for testing, then obtain a mapping between original identifiers and minified identifiers, and then compute accuracy by computing the number of identifier recovered \emph{exactly}. If a particular local variable or function name appears multiple times in the program, it is included only once while computing the accuracy. Global names and property names (which are not minified) are excluded while computing the accuracy.

\begin{table}
    \centering
    \begin{tabular}{|c|c|}
     \hline
     Parameter          &  Value \\
     \hline
     $n_{neighbours}$   &  3\\
     $n_{usages}$       &  5\\
     $vocab_{inp}$      &  4096\\
     $vocab_{out}$      &  60000\\
     $size_{embedding}$ &  80\\
     $size_{hidden}$    &  3500\\
     \hline
    \end{tabular}
    \caption{Network Parameter Values}
    \label{tab:network-params}
\end{table}

\subsection{Comparison with JSNice and JSNaughty}
To compare our tool with JSNice and JSNaughty, we first train these two tools on our training dataset. There are multiple versions of the JSNice system available. The most commonly used is the web-interface \footnote{\url{http://jsnice.org}}, but the underlying implementation is not available. We instead use the implementation provided in the artifact accompanying the JSNice paper, as it can be trained on a custom dataset. For JSNaughty, we use the docker implementation, for which they provide instructions on their Github page. We then evaluate all the tools on the testing dataset using the metric described in Section \ref{sec-evaluation-setup}.

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
     Tool        & Accuracy & Average Prediction Time (seconds)  \\
     \hline
      Us         & 60.2\%     & ?? \\
      JSNice     & 49.6\%     & ?? \\
      JSNaughty  & ??         & ?? \\
      \hline
    \end{tabular}
    \caption{Comparison with JSNice and JSNaughty}
    \label{tab:comparison-using-metric-1}
\end{table}

Table \ref{tab:comparison-using-metric-1} summarizes the accuracy of each tool, along with prediction time averaged over all minified local names across all the files. The data suggests that our tool performs significantly better than JSNice, and is equally efficient. \texttt{Insert comment on JSNaughty's accuracy}. JSNaughty has worse running times, which the authors attribute to the large phrase tables that need to be loaded and queried in the prediction phase.

==> introduction.tex <==
\section{Introduction}
Developers invest a significant portion of their time in reading and understanding code \cite{Singer1997}. This is because programmers need to periodically review their code for defects, to look for regions of code to optimize, extend existing functionality or simply increase their knowledge base \cite{Bacchelli2013}. The developer community has come up with various guidelines and styles to be followed while writing programs which can potentially reduce the comprehension overhead. One widely accepted guideline is to use meaningful variable and function names. Ideally, a name should capture its semantic function in a program, effectively acting as an abstraction which developers can use to aid their understanding \cite{Gellenbeck1991}.

In the same vein, however, variable and function names when deliberately designed poorly, can provide a layer of obfuscation that discourages review and inspection. This when combined with the removal of formatting, such as indentation and white-spaces, while retaining functionality, can make a program much smaller and extremely difficult to read for a developer. An especially pertinent use-case is JavaScript. Modern websites extensively use JavaScript to provide a richer experience to users, and is passed along with the website content when a user requests a web-page. Thus, smaller JavaScript files would reduce the download time and the bandwidth usage. In addition to this, the developers of the website might wish to conceal the semantic meaning of the code for protection of their intellectual property or owing to their malicious intent. A number of publicly available tools automate this obfuscation process by \emph{mangling} local names to short cryptic ones, and aggressively reusing them in different scopes. One such popular tool is \texttt{UglifyJS}\footnote{\url{https://github.com/mishoo/UglifyJS2}}. Figure \ref{fig:uglifyjs-example}XXX shows a JavaScript code snippet before and after being subjected to minifaction by \texttt{UglifyJS}.

Automated minifiers usually produce \emph{source-maps}, which provide information on mapping various elements in the minified code back to their original counterparts. Unfortunately, in most cases source-maps are available only to the authors of the JavaScript code as they are not shipped along with the source. To enable external reviewing and security analyses, it is important to develop techniques that attempt to recover original source code from its minified version, primarily by renaming identifiers to more meaningful names.

The idea is to leverage the huge amount of JavaScript code that is available online, by extracting useful naming patterns and their correlation with the semantic function of these names within the program. Machine learning techniques exploiting this availability of source code have been used to solve a variety of development tasks, such as fixing syntactic errors \cite{Gupta2017}, code clone detection \cite{White2016}, malware analysis \cite{David2015} and even generating programs with specific constraints \cite{Shu2017}. Deep Learning \cite{LeCunn2015DPL} is a fast-growing field in machine learning that has been very successful in natural language tasks such as completion, translation and summarization. We show that this effectiveness propogates to the domain of source code as well.

We introduce a new technique based on deep learning that is able to predict natural names for these mangled identifiers that capture their semantic function in the program. We validate our claim by showing evaluating our technique on a large, publicly available corpus of JavaScript source code (not minified), wherein our tool is able to recover XXX\% of the identifiers \emph{exactly} i.e. our tool predicts the \emph{same} name that the authors of the original programs had in mind for XXX\% of the identifiers. We also show that our approach is practical - our tool takes an average of XXX ms to process a XXXXXXXXXX \textit{(not sure how to report this yet)}. For comparison, we evaluated the existing tools JSNice \cite{Raychev2015} and JSNaughty \cite{Vasilescu2017} on the same dataset. The tools were able to recover XXX\% and XXX\% of the identifiers respectively. This indicates that our technique improves the state-of-the-art by XXX\%.

The key idea in our approach is to capture the usage of variable or function across a JavaScript program as a sequence of lexical tokens, compiled from the tokens surrounding every use of that variable/function. This essentially represents the syntactic context around every use of that variable/function. We can use these sequences to train a \emph{recurrent neural network} (RNN) to predict a natural identifier which summarizes this context, which should correspond to summarizing its usage. However, since these sequences can be arbitrarily long, we use a separate \emph{autoencoder} network to generate \emph{embeddings}, which are much smaller in dimensionality, and retain the key features that are sufficient to categorize these sequences. The RNN used for prediction can be trained much more efficiently with these embeddings.

This paper makes the following contributions - 
\begin{itemize}
    \item A deep learning framework to recover natural identifier names from minified JavaScript code.
    \item Our tool XXX based on this framework, that is able to recover XXX\% of the minified names \emph{exactly} from a large, publicly available corpus of JavaScript programs, which improves over the state-of-the-art by XXX\%.
\end{itemize}

==> overview.tex <==
\section{Overview}
In this section, we present an informal outline of our approach on a concrete minified JavaScript program. Figure \ref{fig:overview} shows the program whose identifiers have been minified using \texttt{UglifyJS}. The local variable names inside the top-level function have been replaced by short non-descriptive names. Note that the function name has not been minified as it is in the global scope. Recovery of natural identifiers for these variable names involves the following phases, executed once for every minified identifier~:\newline

\noindent\textbf{Extracting Usage Context :} We convert the input JavaScript program into a stream of lexical tokens. For every occurrence of the token corresponding to the target minified variable in its respective scope, we extract neighbouring tokens and aggregate them into a single sequence. This sequence represents the structure immediately surrounding the various points of usage of that identifier. We limit the size of this sequence by imposing a ceiling on the number of occurrences of the target token to consider.\ksen{This part is quite informal and I was unbale to follow with precision. In this section one should not focus how to do things, rather the focus should be why we do things this way.}\newline

\noindent\textbf{One-hot encoding :} We now need to process this usage sequence in order to be able to train the network efficiently. Since the number of possible tokens is infinite because of the presence of global identifiers, we define an vocabulary of tokens that the network understands, called the input vocabulary. Tokens are outside this vocabulary are casted as \texttt{UNKNOWN} tokens. We use this vocabulary to transform each token into its one-hot representation i.e. a binary vector of length equal to the vocabulary size, and with the $i^th$ bit set if the token under question occupies the $i^th$ position in the vocabulary. \newline

\noindent\textbf{Embedding Generation :} The dimensionality of this sequence has now increased by as many times as the input vocabulary size! To represent this sequence more efficiently, and to discard possible redundant information, we use an autoencoder network to convert this sequence into a sequence of embeddings which are of much smaller dimensionality, and capture enough information to be able to reproduce the the original large sequence with high accuracy.\newline

\noindent\textbf{Prediction :} This sequence of embeddings is now fed to a recurrent neural network (RNN), which outputs a probability distribution over an output vocabulary, which is a vocabulary of natural identifier names. We then finally emit the name in the vocabulary with the highest probability as the final prediction for the target minified variable.\newline

It is interesting to note that the prediction given for the variable XXX in figure \ref{fig:overview} nicely summarizes its utility within the program, and matches the developer's intent in the original program given in figure XXX.


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/overview.png}
    \caption{Overview of our technique (Incomplete)}
    \label{fig:overview}
\end{figure*}



==> related-work.tex <==
\section{Related Work}

==> technical-details-v2.tex <==
\section{Technical Details - Version 2}
In this section, we provide the technical details of our approach. We capture the \emph{usage} of a variable or function across a program as a sequence of lexical tokens, which we define as a \emph{usage sequence}. \ksen{Define a usage sequences first before using it. In general, define every term before you use the term.} This sequence approximates the semantic meaning of the variable or function in the program. We can then train a recurrent neural network (RNN) to predict natural identifier names based on these usage sequences. 

The first part (Sec. \ref{sec-usage-sequence}) specifies our construction of usage sequences for variables and functions. The second part (Sec. \ref{sec-embedding}) describes the how we can obtain a compact representation (embeddings) of such usage sequences using an RNN-based autoencoder. Finally, the third part (Sec. \ref{sec-lstm}) describes our RNN-based predictor which takes this sequence of embeddings as the input and gives a prediction for a suitable identifier name.

%-------------------------------------
% Subsection : Usage Sequences
%-------------------------------------

\subsection{Usage Sequence}\label{sec-usage-sequence}
\ksen{The formalism looks good, but it is unnecessarily detailed. We should not introduce any notation that we are not using.  For example, I do not see any usage of the scopes $s_i$s.  The goal of writing would be introduce minimal number of notations while making sure the description precise and easy to follow.}
Our notion of a usage sequence closely resembles that of a \emph{usage representation} in \cite{Allamanis2017}. We view the JavaScript source as a sequence of lexical tokens $\mathcal{T} = <t_0, t_1, \cdots , t_n>$. Let $\mathcal{I} = \{(i_1, s_{i_1}), (i_2, s_{i_2}), \cdots , (i_n, s_{i_n})\}$ be the set of all pairs $(i, s_i)$ in the program, where $i \in \mathcal{T}$ is a local identifier name \ksen{what is a "local" identifier name?} (variable name or function name), and $s(i)$ \ksen{what is $s(i)$? do you mean $s_i$?} is its corresponding scope.

Let $\mathcal{T}[k]$ denote the $k^{th}$ token in the sequence $\mathcal{T}$. We define a token retrieval function $g_\mathcal{T}$ for $\mathcal{T}$ as follows -
\begin{equation}
    g_\mathcal{T}(k) = \begin{cases}
               \mathcal{T}[k] \text{ if } 0 \leq k \leq n\\
               \text{START} \text{  if } k < 0\\
               \text{END} \text{  if } k > n
             \end{cases}
\end{equation}
Note that $g_\mathcal{T}$ returns special boundary tokens \texttt{START} and \texttt{END}, if its argument is out of range. We define the context $c(k)$ of the $k^{th}$ token in $\mathcal{T}$ as follows: \ksen{What is $C$ here?} 

\begin{align}
\begin{split}
    c(k) = < & g_\mathcal{T}(k-C), \cdots, g_\mathcal{T}(k-1), \\
           & g_\mathcal{T}(k+1), \cdots, g_\mathcal{T}(k+C)> \\
\end{split}
\end{align}

The context $c(k)$ of the token $\mathcal{T}[k]$ is a sequence of $C$ tokens before and $C$ tokens after $\mathcal{T}[k]$. $C$ is a tunable hyper-parameter in our framework. Let $\mathcal{P}(i, s_i, k)$ represent the index corresponding to the $k^{th}$ occurrence of the token \ksen{"the token": which token are you referring to?} in $\mathcal{T}$, corresponding to the identifier $i$ in scope $s_i$. If no such index exists, $\mathcal{P}(i, s_i, k) = -1$. 

We can now define a usage sequence composed of $L$ contexts, for a pair $(i, s_i) \in \mathcal{I}$ as follows - 

\begin{align}
\begin{split}
    u(i, s_i, L) & = \begin{cases}
                        c(k) \circ u(i, s_i, L-1) \text{ if } k = \mathcal{P}(i, s_i, L) \land k \neq -1\\
                        \omega \circ u(i, s_i, L-1) \text{ if } k = \mathcal{P}(i, s_i, L) \land k = -1\\
                   \end{cases}\\
    where \\
    \omega & = \underbrace{<\text{PAD ,} \cdots \text{, PAD}>}_{2C \text{ times }}
\end{split}
\end{align}

$L$ is another hyper-parameter in our framework, which bounds the size of the usage sequence. The $\circ$ operator combines two or more sequences. Notice that we pad the usage sequence with a context made up of special \texttt{PAD} tokens when there are not enough occurrences of the identifier corresponding to $(i, s_i)$, to fix its size.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/usage-sequence.png}
    \caption{Usage sequence construction (PROTOTYPE)}
    \label{fig:usage-sequence}
\end{figure*}

\subsubsection{Preparing RNN-friendly Inputs}
In their current form, usage sequences can be arbitrarily long, proportional to the number of usages of an identifier. Moreover, the tokens are strings which can be of arbitrary length as it includes global names. Training RNNs on such variable data is very hard, and networks have been shown to perform poorly. 

We first normalize all usage sequences to a fixed length, by defining a parameter $n_{usages}$. During construction of a usage sequence for a local identifier, we only consider the first $n_{usages}$ occurrences of the identifier. For the example in figure \ref{fig:usage-sequence}, if the value of $n_{usages}$ is 2, only the first two occurrences of the local identifier name \texttt{a} would be considered, and the usage sequence would consist of only 12 tokens. If the number of occurrences is less than $n_{usages}$, we pad the sequence with $(n_{usages} - n) \times (n_{neighbours} \times 2)$ custom ``PAD'' tokens where $n$ is the actual number of occurrences of the identifier.

We then normalize the size of each token to a fixed length in these sequences, by first defining an \emph{input vocabulary} of size $vocab_{inp}$, and then converting each token into its \emph{one-hot encoding} based on this vocabulary. The input vocabulary dictates the tokens our network is able to uniquely identify. For this, we take the most frequent $vocab_{inp} - 4$ tokens (excluding all the custom tokens) over the entire training dataset, and include them in the vocabulary. We then add the custom tokens \texttt{START}, \texttt{END}, \texttt{PAD}, along with another token \texttt{UNKNOWN}, which represents any token outside the vocabulary. We then convert each token into its \emph{one-hot encoding} based on its position in this vocabulary. The one-hot encoding of the $i^{th}$ token in this vocabulary is a binary vector of length $vocab_{inp}$, with all but the $i^{th}$ bit off. We prefer one-hot encodings over normal integer encodings as integer encodings inherently establish an ordering between the various elements, which is not appropriate in our setting over tokens. Finally, we have an RNN-friendly usage sequence representation as a binary vector of length $(vocab_{inp} \times n_{neighbours} \times n_{usages} \times 2)$.

%-------------------------------------
% Subsection : Embeddings for Usage Sequences
%-------------------------------------

\subsection{Embeddings for Usage Sequences}\label{sec-embedding}
The last section described how a usage sequence is converted into a binary vector of size proportional to the size of the vocabulary of tokens. There is an inherent conflict here - on one hand, we would like the vocabulary to be large, so the network is able to distinguish between more tokens, but on the other hand, we would also like our input to the final prediction network to be smaller to reduce memory usage as well as improve training and prediction times. 

An Autoencoder is a neural network trained to reconstruct its own input at the output layer. Internally, the autoencoder has a number of hidden layers, which are mostly lower in dimensionality than the input/output layers. Overall the network may be partitioned into two parts - the encoder function $f(i)$ which produces an embedding $h$ for the input $i$, and a decoder function $d(h)$ which takes this embedding $h$ and attempts to reproduce $i$. If the the size of the encoding is sufficiently small, and the network is given enough examples, the encoder learns to extract useful features from the input, and use them to categorize the input uniquely, which is enough for the decoder to reproduce the input.

We use an autoencoder (specifically, the encoder component) to reduce the size of the usage sequence input. This serves a dual purpose - it reduces the size of the prediction network itself, and it also extracts salient features from the sequence to be focused on. We construct embeddings for every sequence of $n_{neighbours} * 2$ tokens corresponding to a \emph{single} usage of an identifier within the usage sequence. We define the size of an embedding as $size_{embed}$. Therefore, we obtain a compressed usage sequence of size $size_{embed} * n_{usages}$. The design of our encoder consists of a single hidden layer comprising of $size_{embed}$ number of \texttt{LSTM} units\ksen{This is not true.  There is only one LSTM unit for the encoder and one for the decoder}. For the decoder, our design consists of a \texttt{Repeat} layer which repeats the output of the encoder $n_{neighbours}$ times, and passes it to another \texttt{LSTM} layer built with $vocab_{input}$ units, whose output is then processed temporally to produce an output sequence of the same size as the input. Essentially, the encoder learns to extract salient features, which, for the decoder, when combined with positional information from the \texttt{Repeat} layer is highly effective in reproducing the input.

A visualization of the network is provided in figure \ref{fig:embedding-network}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/embedding_model.png}
    \caption{Embedding RNN (Placeholder)}
    \label{fig:embedding-network}
\end{figure}

%-------------------------------------
% Subsection : Natural Identifier Prediction
%-------------------------------------

\subsection{Natural Identifier Prediction}\label{sec-lstm}
We now describe our main RNN which takes these sequences comprising of $n_{usages}$ number of embeddings, each of size $size_{embed}$, and outputs a prediction for a suitable identifier name. The network consists of an input layer, followed by a single hidden layer comprising of $size_{hidden}$ number of \texttt{LSTM} units\ksen{again there is a single LSTMCell}, whose output is passed to a final \texttt{softmax} layer which makes the prediction. The size of the softmax layer is governed by the \emph{output vocabulary} for this RNN, which represents the output space of the network. Its size is denoted by $vocab_{out}$. The vocabulary is constructed by picking the most frequent $vocab_{out} - 1$ tokens corresponding to local identifier names, along with the \texttt{UNKNOWN} token to represent tokens outside this vocabulary. The softmax layer outputs a probability distribution over this output vocabulary, wherein the element with the highest probability corresponds to the prediction. A visualization of the network is provided in figure \ref{fig:prediction-network}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/lstm_model.png}
    \caption{Prediction RNN (Placeholder)}
    \label{fig:prediction-network}
\end{figure}

%-------------------------------------
% Implementation
%-------------------------------------

\section{Implementation}
\subsection{Training}\label{sec-impl-training}
We now summarize the training phase for our tool. We use a large corpus of non-minified JS files. We then minify these files using a popular off-the-shelf minifier, and also obtain a mapping between minified identifier names and the original identifier names for each file. We extract usage sequences for each local identifier in the minified files, and then train an autoencoder on these usage sequences, whose encoder component is used to convert them into sequences of embeddings. These sequence of embeddings is then used to train the prediction RNN, with the target output being the original, non-minified identifier name, which can be obtained using the map.

\subsection{Prediction}
For getting predictions, we simply extract usage sequences for every local identifier from the input minified JS file, pass them to the encoder to obtain sequences of embeddings, and finally feed them into the prediction RNN to recover natural identifier names.


==> technical-details.tex <==
\ksen{The following section seems to be repetition of section 3.}
\section{Technical Details}
In this section, we describe our technique based on deep learning to recover natural identifier names from minified JS programs. The idea is to capture the \emph{usage} of a variable or function across a program as a sequence of tokens, which we define as a \emph{usage sequence}. We can then train a recurrent neural network (RNN) to predict natural identifier names based on these usage sequences. 

The first part (Sec. \ref{sec-usage-sequence}) specifies our construction of usage sequences for variables and functions. The second part (Sec. \ref{sec-embedding}) describes how we can obtain a compact representation (embeddings) of such usage sequences using an Autoencoder RNN. Finally, the third part (Sec. \ref{sec-lstm}) describes our RNN which takes this sequence of embeddings as the input and gives a prediction for a suitable identifier name as the output.

%-------------------------------------
% Subsection : Usage Sequences
%-------------------------------------

\subsection{Usage Sequence}\label{sec-usage-sequence}
We define a configurable parameter $n_{neighbours}$. This parameter dictates the size of a usage sequence. The construction of a usage sequence involves multiple steps - 
\begin{itemize}
    \item Convert the input minified JS program into a list of tokens. Whitespace and comments are ignored.
    \item Prepend $n_{neighbours}$ copies of a custom token ``START'', and append $n_{neighbour}$ copies of a custom token ``END'' to this list.
    \item Drop all tokens corresponding to punctuators (.) and round brackets.
    \item For every occurrence of a local identifier token corresponding to a unique local variable or a local function, take $n_{neighbours}$ number of preceding tokens and $n_{neighbours}$ number of following tokens, and aggregate them into a single sequence.
    \item Replace every instance of a local identifier with the custom token ``ID''.
    \item This sequence corresponds to the usage sequence for the unique local variable or function.
\end{itemize}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/usage-sequence.png}
    \caption{Usage sequence construction (PROTOTYPE)}
    \label{fig:usage-sequence}
\end{figure*}

\noindent Essentially, we are describing the usage of a local identifier based on the tokens surrounding every occurrence of that identifier. This process is illustrated in Figure \ref{fig:usage-sequence}, which shows an example of a minified program with one local variable \texttt{a}, which is an argument of the global function \texttt{negate} whose name is not minified. The parameter $n_{neighbours}$ is set to a value of \texttt{3}. We then obtain a usage sequence for \texttt{a}, comprising of 18 tokens.

\subsubsection{Preparing RNN-friendly Inputs}
In their current form, usage sequences can be arbitrarily long, proportional to the number of usages of an identifier. Moreover, the tokens are strings which can be of arbitrary length as it includes global names. Training RNNs on such variable data is very hard, and networks have been shown to perform poorly. 

We first normalize all usage sequences to a fixed length, by defining a parameter $n_{usages}$. During construction of a usage sequence for a local identifier, we only consider the first $n_{usages}$ occurrences of the identifier. For the example in figure \ref{fig:usage-sequence}, if the value of $n_{usages}$ is 2, only the first two occurrences of the local identifier name \texttt{a} would be considered, and the usage sequence would consist of only 12 tokens. If the number of occurrences is less than $n_{usages}$, we pad the sequence with $(n_{usages} - n) \times (n_{neighbours} \times 2)$ custom ``PAD'' tokens where $n$ is the actual number of occurrences of the identifier.

We then normalize the size of each token to a fixed length in these sequences, by first defining an \emph{input vocabulary} of size $vocab_{inp}$, and then converting each token into its \emph{one-hot encoding} based on this vocabulary. The input vocabulary dictates the tokens our network is able to uniquely identify. For this, we take the most frequent $vocab_{inp} - 4$ tokens (excluding all the custom tokens) over the entire training dataset, and include them in the vocabulary. We then add the custom tokens \texttt{START}, \texttt{END}, \texttt{PAD}, along with another token \texttt{UNKNOWN}, which represents any token outside the vocabulary. We then convert each token into its \emph{one-hot encoding} based on its position in this vocabulary. The one-hot encoding of the $i^{th}$ token in this vocabulary is a binary vector of length $vocab_{inp}$, with all but the $i^{th}$ bit off. We prefer one-hot encodings over normal integer encodings as integer encodings inherently establish an ordering between the various elements, which is not appropriate in our setting over tokens. Finally, we have an RNN-friendly usage sequence representation as a binary vector of length $(vocab_{inp} \times n_{neighbours} \times n_{usages} \times 2)$.

%-------------------------------------
% Subsection : Embeddings for Usage Sequences
%-------------------------------------

\subsection{Embeddings for Usage Sequences}\label{sec-embedding}
The last section described how a usage sequence is converted into a binary vector of size proportional to the size of the vocabulary of tokens. There is an inherent conflict here - on one hand, we would like the vocabulary to be large, so the network is able to distinguish between more tokens, but on the other hand, we would also like our input to the final prediction network to be smaller to reduce memory usage as well as improve training and prediction times. 

An Autoencoder is a neural network trained to reconstruct its own input at the output layer. Internally, the autoencoder has a number of hidden layers, which are mostly lower in dimensionality than the input/output layers. Overall the network may be partitioned into two parts - the encoder function $f(i)$ which produces an embedding $h$ for the input $i$, and a decoder function $d(h)$ which takes this embedding $h$ and attempts to reproduce $i$. If the the size of the encoding is sufficiently small, and the network is given enough examples, the encoder learns to extract useful features from the input, and use them to categorize the input uniquely, which is enough for the decoder to reproduce the input.

We use an autoencoder (specifically, the encoder component) to reduce the size of the usage sequence input. This serves a dual purpose - it reduces the size of the prediction network itself, and it also extracts salient features from the sequence to be focused on. We construct embeddings for every sequence of $n_{neighbours} * 2$ tokens corresponding to a \emph{single} usage of an identifier within the usage sequence. We define the size of an embedding as $size_{embed}$. Therefore, we obtain a compressed usage sequence of size $size_{embed} * n_{usages}$. The design of our encoder consists of a single hidden layer comprising of $size_{embed}$ number of \texttt{LSTM} units. For the decoder, our design consists of a \texttt{Repeat} layer which repeats the output of the encoder $n_{neighbours}$ times, and passes it to another \texttt{LSTM} layer built with $vocab_{input}$ units, whose output is then processed temporally to produce an output sequence of the same size as the input. Essentially, the encoder learns to extract salient features, which, for the decoder, when combined with positional information from the \texttt{Repeat} layer is highly effective in reproducing the input.

A visualization of the network is provided in figure \ref{fig:embedding-network}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/embedding_model.png}
    \caption{Embedding RNN (Placeholder)}
    \label{fig:embedding-network}
\end{figure}

%-------------------------------------
% Subsection : Natural Identifier Prediction
%-------------------------------------

\subsection{Natural Identifier Prediction}\label{sec-lstm}
We now describe our main RNN which takes these sequences comprising of $n_{usages}$ number of embeddings, each of size $size_{embed}$, and outputs a prediction for a suitable identifier name. The network consists of an input layer, followed by a single hidden layer comprising of $size_{hidden}$ number of \texttt{LSTM} units, whose output is passed to a final \texttt{softmax} layer which makes the prediction. The size of the softmax layer is governed by the \emph{output vocabulary} for this RNN, which represents the output space of the network. Its size is denoted by $vocab_{out}$. The vocabulary is constructed by picking the most frequent $vocab_{out} - 1$ tokens corresponding to local identifier names, along with the \texttt{UNKNOWN} token to represent tokens outside this vocabulary. The softmax layer outputs a probability distribution over this output vocabulary, wherein the element with the highest probability corresponds to the prediction. A visualization of the network is provided in figure \ref{fig:prediction-network}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/lstm_model.png}
    \caption{Prediction RNN (Placeholder)}
    \label{fig:prediction-network}
\end{figure}

%-------------------------------------
% Implementation
%-------------------------------------

\section{Implementation}
\subsection{Training}\label{sec-impl-training}
We now summarize the training phase for our tool. We use a large corpus of non-minified JS files. We then minify these files using a popular off-the-shelf minifier, and also obtain a mapping between minified identifier names and the original identifier names for each file. We extract usage sequences for each local identifier in the minified files, and then train an autoencoder on these usage sequences, whose encoder component is used to convert them into sequences of embeddings. These sequence of embeddings is then used to train the prediction RNN, with the target output being the original, non-minified identifier name, which can be obtained using the map.

\subsection{Prediction}
For getting predictions, we simply extract usage sequences for every local identifier from the input minified JS file, pass them to the encoder to obtain sequences of embeddings, and finally feed them into the prediction RNN to recover natural identifier names.

